CFEAR Radarodometry -- Conservative Filtering for Efficient and Accurate Radar Odometry

This paper presents the accurate, highly efficient, and learning-free method CFEAR Radarodometry for large-scale radar odometry estimation. By using a filtering technique that keeps the k strongest returns per azimuth and by additionally filtering the radar data in Cartesian space, we are able to compute a sparse set of oriented surface points for efficient and accurate scan matching. Registration is carried out by minimizing a point-to-line metric and robustness to outliers is achieved using a Huber loss. We were able to additionally reduce drift by jointly registering the latest scan to a history of keyframes and found that our odometry method generalizes to different sensor models and datasets without changing a single parameter. We evaluate our method in three widely different environments and demonstrate an improvement over spatially cross-validated state-of-the-art with an overall translation error of 1.76% in a public urban radar odometry benchmark, running at 55Hz merely on a single laptop CPU thread.

==> backup/introduction_backuo.tex <==
%Determining if point clouds are correctly aligned is essential to enable robust mobile robotics. Applications such as mapping, scene understanding and sensor calibration are prone to miss alignment of point clouds and requires capability to asses reliability of scan alignment used in the process to avoid devastating failures. Alignment error occurs due to uncompensated motion distortion or wrong convergence in the scan registration.  Our system: ``CorAl'' can detect both these type of errors in real-time, even with small alignment errors. 
%Our method  is well grounded in information theory which and we provide an intuitive formulation of the problem. CorAl measures the difference between the entropy of the merged and separate point clouds and can be used to detect miss alignment. For aligned point clouds, the merged cloud and separate point clouds are similarly blured which provides a measure close to zero. In contrast, merged misaligned point clouds tend to ``blur'' the scene which can be observed by the increase in entropy. The separate point clouds are used to discount for the entropy of the scene. Consequently, the measure provides an absolute understanding of the alignment reliability.\\\\


In order to create safe and efficient mobile robots, introspective capabilities are required to assess and recover from perception failures. Various perception tasks, including localization~\cite{zhang_loam_2014,adolfsson_submap_2019}, scene understanding and sensor calibration~\cite{della_corte_unified_2019}, rely on point cloud registration. However, registration may provide incorrect estimates due to wrong convergence, uncompensated motion distortion, sensor noise or lack of features~\cite{andreasson_incorporating_2017}, potentially causing a system failure or hazard. Consequently, it is essential that the quality of registration is assessed, and unsuccessful attempts are rejected or re-estimated.

In the past, various methods have been proposed to assess the alignment quality of point cloud pairs. One category of methods attempts to provide an uncertainty estimate between point clouds~\cite{David_Landry,bengtsson_robot_2003, nieto_scan-slam_2006,prakhya_closed-form_2015}. However, these methods rely on the assumption that the registration has reached a global maximum -- which may be invalid --  and cannot be used to assess absolute alignment quality.

%perhaps more expli
More recently, Almqvist et al. presented a learning approach to detect misaligned point clouds ~\cite{Almqvist}. A strong classifier was trained based on weaker classifiers derived from common point cloud measures~\cite{rusinkiewicz-2001-fasticp,biber_normal_2003,magnusson-2009-phd,chandran-ramesh_assessing_2007,makadia-2006-fully,silva-2005-ga}.
%~\cite{akai_misalignment_2019,biber_normal_2003, stoyanov_comparative_2013, magnusson-2009-phd}. 
The classifiers were evaluated on two outdoor data sets, and although the combined classifier, as well as some of the individual ones, reach almost 90\,\% classification accuracy for the hardest cases on each data set individually, accuracy dropped to around 80\,\% when cross-evaluating between the data sets.
%The authors reported significantly reduced classification accuracy for all evaluated classifiers when applied to new environments. A key reason for the lack of robustness to environmental changes is that current classifiers do not account for the appearance of the environment and rely heavily on parameter tuning.\\

%Alqvist writes that ``we hope that more specific classifiers will be investigated''.
%Work by  Chandran-Ramesh and Paul Newman ~\cite{chandran-ramesh_assessing_2007} later adopted to pointcloud-pairs by almqvist
%akai_misalignment_2019 detect localization error.
%ICP COVARIANCE Monte Carlo: bengtsson_robot_2003
% closed form ~\cite{nieto_scan-slam_2006}.
% closed formprakhya_closed-form_2015
%useful for pose-graph optimization.
In this paper, we propose ``CorAl'': an accurate and fast  alignment measure and binary classifier for point cloud pairs to bridge the gap in classification performance when the method is applied in new unseen environments without retraining.

% both these type of errors in real-time, even with small alignment errors. CorAl 
Our method is well grounded in information theory and gives an intuitive formulation to the alignment quality problem. CorAl measures the difference between the entropy of the merged and separate point clouds. For well-aligned point clouds, the merged cloud and separate point clouds
have similar entropy %are similarly blured 
and provide a measure close to zero. In contrast, misaligned point clouds tend to ``blur'' the scene which can be observed by an increase in entropy. The separate point clouds are used to discount for the entropy inherent in  the scene. Consequently, the measure provides an absolute understanding of the alignment quality. 





%This work is related to large-scale localization and mapping. THere are multiple essential parts in such system and depending on the application requirements they techniques may vary significantly. Many localization problems are related to finding the alignment between point clouds. If the relative alignment is known, the motion or the location of the robot has been determined. Most systems find the alignment by making assumptions on the quality and relative alignment of point clouds and then deploy well established methods from mathematics to solve the alignment. If any of these assumptions are violated, the localization is likely to fail. For example. Most lidar odometry systems uses the motion of the wheel of the robot to compensate for distortion in the data. based on this correction, local registration methods are used to find the relative alignment. This scenario is likely to introduce two different errors, at least to some extent. The first error is that the motion compensation is inaccurate due to slippage, unsyncronized sensors or noise. This causes the data be inaccurate. The second problem depend on that local registration methods have a limited convergence basin. The registration can fail if the initial alignment is not sufficiently close to the true solution. If the localization algorithms is able to detect occurance of such problems, it can likely also be build to manage and recover from them. Thus making more robust localization systems for robots.

The contribution of this paper is an intuitive and simple measure of the absolute alignment quality between pairs of point clouds based on a relative change in scene entropy. We demonstrate how to use this quality measure to learn to detect misaligned point clouds and how to utilize our tool for manual inspection of alignment quality.
We provide an open source ROS/C++ implementation\footnote{https://github.com/dan11003/CorAl-ScanAlignmentClassification} and make our evaluation available to the community. 

We make the following claims: (i) Our proposed measure provides an absolute understanding of alignment quality by accounting for the expected scene entropy. 
(ii) Our method is highly accurate in %specific environments, 
a wide range of environments and %can even improve adaptation to new unseen environments compared to state-of-the-art alignment classification.
generalizes well to new environments without retraining.





%Fig.~\ref{fig:example_1} 


==> backup/related_work_backup.tex <==
 
Various methods have been used to assess alignment quality. Traditional methods calculate the root mean squared (RMS) point-to-point error, which also is the function that
is minimised by iterative closest point (ICP) registration~\cite{ICP}, or a point-to-distribution~\cite{ndtbiber} distance.
%The minimization is typically stopped when a local minima is found or a maximum number of iterations are reached.
As reported in Almqvist et al.~\cite{Almqvist}, the absolute level of score is sensitive to method parameters, environment and sensing noise. Consequently, they are  are poorly suited for global alignment classification. 

A family of methods attempts to estimate the alignment uncertainty between point cloud pairs. 
Some use Monte Carlo strategies to estimate uncertainty by sampling registrations in a region. This exhaustive search is however unpractical in mobile robotics.
Other attempt to estimate uncertainty in closed form using the Hessian, representing the steepness of the alignment score function around a local minima. These methods assumes correct alignment as they are fundamentally limited by the traditional alignment scores. Consequently, the uncertainty estimation and cannot give an absolute alignment quality. 

Almqvist et al.~\cite{Almqvist} extensively explored building classifiers based on the traditional RMS and Point-to-distribution (P2D) scores. 
The authors also derived a classifier based on Chandran-Ramesh and Newman~\cite{chandran-ramesh_assessing_2007}, which attempts to find suspicious regions in the map, counting planar intersections. The authors proposed AdaBoosting for fusing and improving the individual classifiers. While this did not have a major impact on the classification accuracy, their method reduced parameter sensitivity. %When evaluating the learned classifiers to new environments, RMS and NDT-P2D scored around 50\% accuracy. %While modifying NDT-P2D showed improved performance.
While RMS and L2 classifiers performed on par with random when transferred into new environments without adjusting parameters.
We notice that this limitation inherits from the traditional distance measures.

Liao et al. \cite{fuzzybnb} recently proposed a global registration method representing point clouds as fuzzy sets. The method first attempts to find a consistent clustering by centering clusters at representative locations. A measure that compares the similarity of points distributions around cluster centers is then used to provide a quality assessment in the absence of ground truth. 
Unlike other global registration methods, the quality assessment is used as a stop criteria to end the global search when a coarse alignment is reached. Afterwards, fine tuning is applied to refine this coarse solution and obtain a precise alignment. 
This quality assessment is not sensitive to small misalignment. Accordingly, we categorize this work as coarse alignment quality assessment. In this work we're interested in fine alignment quality assessment.
%%The argument of this quality assessment builds on the robustness of the fuzzy center points. When wil this perform and when will it not?
%As the clustering comes with a high complexity, the method is intractable without downs
Additionally, the method requires at least 50\% overlap between the point clouds which may not be possible in mobile robotic applications. 
Our methods does not require a minimum overlap by operating principle, however we consider point clouds with less than 10\% overlap to provide insufficient evidence to determine alignment quality.\\
%WHy not calculate standard error to determine if there exists evidence for overlap????? 
To the best of our knowledge, there is no method for binary classification of point clouds alignment that performs accurate in real-time and adapts well to new environments.\\

The rest of the paper is structured as follows:
In section \ref{sec:method} we describe our alignment measure and how to train it for binary classification. In section \ref{sec:eval} we propose a benchmark test for further research in the area and evaluate our method on publicly available data.
%https://github.com/zgojcic/3DSmoothNet deep learning high recall
%  Chandran-Ramesh and Paul Newman 

%Introduction
%relative alignment  - local registration
% icp - rms
% ndt - l2 distance
% limited convergence basin - unsuitable for quality assesment
% Broad convergence basin Efficient Global Optimization

%


%Global typically costly, for offline.

%ICP measure%A method for registration of 3-D shapes
%Alqvist et al. \cite{Almqvist} uses AdaBoost to improve a set of weak classifiers.

%Similar covariance estimation}

==> figures/Parameters/figure_k_threshold.tex <==
\begin{tikzpicture}
	\begin{axis}
	[
		width   = 0.95\columnwidth,
		height  = 0.6\columnwidth,
		xmin		= 0,
		xmax		= 90,
		ymin		= 2,
		%ymax		= 0.05,
		%ytick	= {0, 0.25, ..., 1},
		xlabel  = {range $[m]$},
		ylabel  = {scaled power},
		ylabel near ticks,
		ymode = log,
		%	ylabel shift			= 2,
		legend style={
		at={(0.5,1.4)},
		anchor= north,
		fill = none,
		draw=none},
		legend columns			= 2,
	]
	\addplot
	[
		white!70!black,
		very thick,
		%only marks,
%		mark size	= 0.02cm,
%		mark			= *,
	]
	table
	[
		x   = range,
		y   = beam,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{measurements};
	%%%
	\addplot
	[
		white!75!black,
		thick,
		dotted,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
	]
	table
	[
		x   = range,
		y   = thr_k,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{strongest $k$ threshold};
	%%%
	\addplot
	[
		white!25!black,
		thick,
		solid,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
	]
	table
	[
		x   = range,
		y   = thr_cfar,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{CFAR threshold};
	%%%
	\addplot
	[
	white!25!black,
	thick,
	dotted,
	%only marks,
	%		mark size	= 0.02cm,
	%		mark			= *,
	]
	table
	[
	x   = range,
	y   = thr_noise,
	]
	{Datasets/export_figure_threshold.txt};
	\addlegendentry{noise threshold};
	\end{axis}
\end{tikzpicture}


==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/Conclusion.tex <==
In this paper we have presented \ac{TITLE}, a radar odometry method that conservatively filters radar data using the $k$ strongest returns and represents the environment by a sparse set of oriented surface points. The oriented surface points can be used to efficiently and accurately perform scan registration by minimizing a point-to-line metric, obtaining outlier robustness using a Huber loss.
Our method is learning-free, requires no training data and can operate well in widely different environments and on different sensor models without changing a single parameter. Best odometry performance is, however, obtained by parameters tailored to the specific sensor and environment.
%We found that conservative filtering can increase odometry accuracy with little impact on accuracy, % and that drift could be mitigated by constraining the latest scan to recent keyframes at the cost of computational time. 
We found that drift can be further reduced by registering the latest scan to a history of key frames jointly, at the expense of computational time. Despite this, we were able to achieve 55~Hz single-thread performance on a laptop CPU, improving SCV state-of-the-art with $1.76$\% overall translation error in a public urban dataset.
%Through qualitative evaluation we found that our method can generalize well between different sensors models and across widely different environments, without changing any parameters.
%Future work will focus on evaluating different loss functions and weighting residuals by surface uncertainty. 
Future work will focus on applying different cost functions.
%different surface models
%different 
%In the future we plan to extend our tracking framework to a local mapping system. We 

%This papers targets the challange of estimating odometry in large-scale environments. 

%Radar has recently become accurate and versatile for large-scale localization.
%Radar is a challenging sensor as it suffers from a large amount of noise, including speckle noise, reflections, saturation and has a wide beam-width.
%Current systems attempts to mitigate the effect by filtering data, by representation data or by robust matching. 
%Top self-supervision to predict keypoints + ICP.
%Top self-supervision to remove noise and matches full radar image.
%Peak detector per azimuth, matching formulated as a weighted least squares.

%Relies on learning which requires ground truth and significant amount of data. Data representation insufficient, doesnt try to model underlying surface.

%My approach. Keep strongest returns over the expected noise level.
%Model the surface as mean+covariance and estimate surface points+normals

%Registration with point-to-line + robustness with Huber loss.

%RQ
%k largest points removes most radar noise
%that point-to-line improves matching compared to point-to-point.





==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/Evaluation.tex <==
In this section we investigate the performance of our method quantitatively on the public Oxford Radar RobotCar Dataset~\cite{RadarRobotCarDatasetICRA2020}, in an urban environment, %a public benchmark dataset from an urban environment 
and qualitatively on two data sets that we collected in non-urban environments (\textit{Kvarntorp mine} and \textit{Volvo test track}), to demonstrate how the method generalises without site and sensor specific parameter tuning. All experiments were carried out on an i7-7700HQ 2.80~GHz laptop CPU, running in a single thread.

%\resizebox{\columnwidth}{%
%\begin{table*}
%\centering
%\begin{tabular}{|l|lllllllll|}
%\hline
% & \multicolumn{7}{c} $parameters$&\\
% \hline
%Dataset & Th & k-strong  &  d &  keyframes s & Res. r & \textbackslash{}theta\_\{max\} & Huber loss $%\delta$ & Key-frame  dist., rot) & sens-dist  \\ 
%\hline
%Kvarntorp mine    & 85  & 12 & 3 & 3       & 3.5 & 0 & 0.1 & (1,5,5)   & 5 \\
%Eskilstuna quarry & 85  & 12 & 3 & 1 $/$ 3 & 3.5 & 0 & 0.1 & (1,5,5)   & 5\\
%Oxford urban      & 65  & 12 & 3 & 3       & 3.5 & 0 & 0.1 & (0.25,5)  & 1 \\                         %\hline
%\end{tabular}
%\end{table*}
%}
%\begin{table*}
%\begin{tabular}{|l|lllllllll|}
%\hline
% & \multicolumn{7}{c} $parameters$&\\
% \hline
%Dataset & Th & k-strong  &  d &  keyframes s & Res. r & \textbackslash{}theta\_\{max\} & Huber loss $%\delta$ & Key-frame  dist., rot) & sens-dist  \\ 
%\hline
%Kvarntorp mine    & 85  & 12 & 3 & 3       & 3.5 & 0 & 0.1 & (1,5,5)   & 5 \\
%Eskilstuna quarry & 85  & 12 & 3 & 1 $/$ 3 & 3.5 & 0 & 0.1 & (1,5,5)   & 5\\
%Oxford urban      & 65  & 12 & 3 & 3       & 3.5 & 0 & 0.1 & (0.25,5)  & 1 \\                         %\hline
%\end{tabular}
%\end{table*}
%}
%The first experiment in the public Oxford Robocar dataset aims to quantitatively assess the performance of our system.



\subsection{Parameters}
\label{ssec:Parameters}
The full set of parameters can be seen in Table~\ref{tab:Parameter}. We tuned the parameters to an urban environment using the sequence \textit{16-13-42} in the Oxford dataset. This sequence is not included in the evaluation set, with the intention to avoid fitting parameters to the specific traffic conditions in one of the evaluated sequences. After the parameter tuning, the exact same parameters were used through all experiments, despite widely different environments and although different radar models with different range resolutions were used.

%
A brief evaluation of the most important parameters (performed on the Oxford dataset) can be seen in Fig.~\ref{fig:parameter_eval}. 
%
The results in Fig.~\ref{fig:keyframe_eval} show that the accuracy can be improved by increasing $s$ (submap keyframes) at the expense of runtime performance. 
%
Fig.~\ref{fig:k_eval} shows the effect of varying the number $k$ of returns in our filtering method.
Using too few ($k<12$) or too many ($k>35$) points negatively impact accuracy, but within the wide range $12\leq k \leq 35$ the method is largely insensitive to $k$.

 \begin{figure}
 \vspace{0.3cm}
  \begin{center}
    \subfloat[
    Increasing the amount of key-frames $s$
    %Using additional key-frames \textit{s}
    reduces the translation error but requires additional processing time. Resample factor is set to $f=3$. ]{\input{figures/Parameters/figure_submap_key_frame}\label{fig:keyframe_eval}}\hfill
    \subfloat[Within a wide range of values of \textit{k}, \ac{TITLE}  is insensitive to the exact value of \textit{k}.
    %A too large  \textit{k} increases false positive
        A too small or too large value, however, reduces translation and rotation accuracy. ]{\input{figures/Parameters/figure_translation_rotation_error}
    \label{fig:k_eval}}\hfill
    \caption{Accuracy/computation time using different parameters.}\label{fig:parameter_eval}
  \end{center}
  \vspace{-0.3cm}
\end{figure}

%\begin{figure}
%\includegraphics[trim={3.5cm 6cm 3cm 5cm},clip,width=0.49\hsize,angle=0]{figures/parameter_eval/submap_s_eval}
%\includegraphics[trim={3.5cm 6cm 3cm 5cm},clip,width=0.49\hsize,angle=0]{figures/parameter_eval/k_strongest}
%\end{figure}

\begin{table}
\centering
%\begin{adjustbox}{width=\hsize}
\begin{tabular}{l|lll}
%& \multicolumn{3}{c}{Dataset}
\\
Parameters & Value          \\    %                   & \textit{Kvarntorp} &  \textit{VolvoCE} & \textit{Oxford}  \\ 
\hline
$k$                              & $12$ \\ %             & $12$                & $12$     \\
Resample factor $f$                     & $1$ \\  %           & $1$                 & $1$       \\
$\zmin$                               & $55$ \\  %          & $55$                & $55$      \\
Resolution $r$                          & $3.5$ \\  %         & $3.5$               & $3.5$   \\
$\theta_\mathrm{max}$                          & $30$ \\    %        & $30$                & $30$     \\
Huber loss    $\mathcal{L}_\delta$      & $0.1$ \\    %       & $0.1$               & $0.1$  \\
Key-frame (dist[m]/rot[deg])            & $1.5/5^\circ$ \\  %          & $1.5/5^\circ$               & $1.5/5^\circ$\\
$s$                        & $3$ \\   %           & $3$                  & $3$      \\
min. sensor distance [m]                 & $5$ \\     %         & $5$                 & $5$ \\
max. sensor distance [m]                & $100$ \\   %         & $100$               & $100$ \\      
\end{tabular}
%\end{adjustbox}
\caption{Full list of parameters. These are used for all datasets and sensors, except when explicitly mentioned in Sec.~\ref{sec:volvo_eval}. }\label{tab:Parameter}
\end{table}


\subsection{Quantitative evaluation in urban environment}
\label{sec:quantitative_eval_sec}
We provide a quantitative evaluation of the odometry accuracy and performance in a large-scale environment with ground truth positioning. The odometry accuracy was measured as proposed in the KITTI odometry benchmark~\cite{Geiger2012CVPR} using the tool~\cite{zhan2019dfvo} that computes the average translation error ($\%$) and rotation error (deg/m) over all sub sequences between $\{100,200, \ldots, 800\}$~m.

We used the public Oxford Radar RobotCar Dataset which was collected with a roof-mounted Navtech CTS350-X \ac{FMCW} radar running at $4$~Hz, configured with a range resolution of $\gamma=4.38$~cm. The dataset contains 32 traversals through a $10$-km urban environment in varied weather, lighting and traffic conditions.

In order to compare our results, we selected the same sequences that were used in the evaluation by Hong~\cite{hong2020radarslam}, both for quantitative evaluation as presented in Tab.~\ref{tab:results} and the visualization in Fig.~\ref{fig:sequences_oxford}. Learning-based methods are compared using their SCV (Spatial Cross Validation). With SCV, test and training datasets are taken from different parts of the environment, rather than selecting the training data from different traverses in the same locations. Without SCV, test and training datasets are not independent since test and training points may be neighbors~\cite{lovelace_geocomputation_2019}.

%For comparison, we report odometry estimates from other methods and sensor modalities. 

As can be seen in Tab.~\ref{tab:results}, \ac{TITLE} produces the lowest per-sequence and mean SCV error with a translation and rotation error of $1.76\%$ and $0.5$~deg/100m, followed by Barnes Dual Cart~\cite{barnes_masking_2020} ($2.78$\%), Hong odometry~\cite{hong2020radarslam} ($3.11$\%), and Cen ~\cite{8460687} ($3.63$\%).
\textit{Barnes Dual Cart}~\cite{barnes_masking_2020} achieves greater mean accuracy ($1.16$\% error) but only when training and evaluating on the same spatial location. When the authors evaluated their methods on places not seen in the training set, the error increased to from $1.76\%$ to $2.78$\%.
\ac{TITLE} provides a $14$\% lower mean odometry error compared to ~\cite{barnes_under_2020} without SCV. The method does not report SCV error in the original publication and it is unclear how well the method generalizes to new nearby locations or environments. 

We therefore argue that \ac{TITLE} method improves state-of-the-art accuracy for sparse methods, but also improves state-of-the-art among all radar odometry methods conditioned on that the evaluation is not biased with spatially overlapping training and evaluation data.


 \begin{figure}
  \vspace{0.2cm}
  \begin{center}
\includegraphics[width=0.89\hsize,trim={0cm 0cm 0cm 2cm},clip,angle=270]{figures/Oxford/Examples/highlight_start_lowres.jpg}\caption{\label{fig:oxford_overview}Incremental radar odometry using the proposed method over a $10$~km sequence from the Oxford dataset. The first and final pose estimate is highlighted and gives an indication of the total aggregated drift. }
  \end{center}
 \vspace{-0.6cm}
\end{figure}

%\begin{figure}
%\minipage{0.32\textwidth}
%\begin{subfigure}%[b]{0.3\hsize}
%  \includegraphics[width=0.3\hsize]{figures/path/10-12-32.pdf}
%  \caption{10-12-32}\label{fig:awesome_image1}
%\end{subfigure}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%\begin{subfigure}%[b]{0.3\hsize}
%  \includegraphics[width=0.3\textwidth]{figures/path/16-13-09.pdf}
%  \caption{16-13-09}\label{fig:awesome_image1}
%\end{subfigure}
%\endminipage\hfill
%\minipage{0.32\textwidth}
% \begin{subfigure}%[b]{0.3\hsize}
%  \includegraphics[width=0.3\textwidth]{figures/path/17-13-26.pdf}
%  \caption{17-13-26}\label{fig:awesome_image2}
%\end{subfigure}

%\endminipage\hfill
%\minipage{0.32\textwidth}
%\begin{subfigure}[b]{0.3\textwidth}
%  \includegraphics[width=0.3\textwidth]{figures/path/18-14-14.pdf}
%  \caption{18-14-14}\label{fig:awesome_image1}
%\end{subfigure}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%\begin{subfigure}[b]{0.3\textwidth}
%  \includegraphics[width=0.3\textwidth]{figures/path/18-15-20.pdf}
%  \caption{18-15-20}\label{fig:awesome_image1}
% \end{subfigure}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%\begin{subfigure}[b]{0.3\textwidth}
%  \includegraphics[width=0.3\linewidth]{figures/path/16-11-53.pdf}
%  \caption{16-11-53}\label{fig:awesome_image2}
%\end{subfigure}
%\endminipage\hfill
%\end{figure}
 \begin{figure*}[]
  \begin{center}
    \subfloat[10-12-32]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/10-12-32.png}\label{fig:10-12-32}}\hfill
    \subfloat[16-13-09]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/16-13-09.png}\label{fig:16-13-09}}\hfill
    \subfloat[17-13-26]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/17-13-26.png}\label{fig:17-13-26}}\\\
    \vspace{-0.2cm}
     \subfloat[18-14-14]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/18-14-14.png}\label{fig:18-14-14}}\hfill
    \subfloat[18-15-20]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/18-15-20.png}\label{fig:18-15-20}}\hfill
    \subfloat[16-11-53]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.32\hsize]{figures/Oxford/Trajectories/16-11-53.png}\label{fig:16-11-53}}
    \caption{Evaluated Oxford sequences using \ac{TITLE}. For qualitative comparison to other methods we refer to ~\cite{hong2020radarslam}.}\label{fig:sequences_oxford}
  \end{center}
  \vspace{-0.3cm}
\end{figure*}


\begin{table*}
\centering
  \begin{adjustbox}{width=\textwidth}

\begin{tabular}{l|ll|lllllllll|l}
              & & & \multicolumn{1}{l}{\textbf{Sequence}}    &                                                                        \\
\textbf{Method} & \textbf{Evaluation} & \textbf{resolution}        & 10-12-32 & 16-13-09 & 17-13-26 & 18-14-14 & 18-15-20 & 10-11-46 & 16-11-53 & 18-14-46 & Mean  & \textbf{Mean SCV}    \\
\hline \\
Visual Odometry  ~\cite{Churchill2012ExperienceBN} & ~\cite{barnes_masking_2020} & N/A   & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        &    $3.78/0.01$ & N/A         \\
%ORB-SLAM2     & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
\hline \\
%LOAM          & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
SuMa (Lidar)~\cite{behley2018rss}  & ~\cite{hong2020radarslam }& N/A  & $1.1/0.3$ & $1.2$/$0.4$ & $1.1/0.3$ & $0.9/0.1$ & $1.0/0.2$  & $1.1/0.3$        & $0.9/0.3$        & $1.0/0.1$        & $1.16/0.3$    & $1.03/0.3$        \\
\hline \\
Cen~\cite{8460687}    &   ~\cite{barnes_masking_2020} & $0.175$& N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & $3.72/0.95$    & $3.63/0.96$       \\
Robust Keypoints~\cite{barnes_under_2020}    &  & $0.346$    & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & $2.05/0.67^*$    & N/A          \\
Barnes Dual Cart~\cite{barnes_masking_2020} & & $0.043$ & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & N/A        & $\bm{1.16/0.3}^*$    &   $2.784/0.85 $\\
Hong odometry~\cite{hong2020radarslam} & &$0.043$ & $2.98/0.8$        & $3.12/0.9$        & $2.92/0.8$        & $3.18/0.9$        & $2.85/0.9$        & $3.26/0.9$        & $3.28/0.9$        & $3.33/1$        & $3.11/0.9$    & $3.11/0.9$      \\
%Ours (ICP)     & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1        & 1    & 1         \\
%Ours (point-to-line) & & & \textbf{1.813/0.575}          & \textbf{1.977/0.595}        & \textbf{1.942/0.612}        & \textbf{1.962/0.616}        & \textbf{2.284/0.677}        & \textbf{1.875/0.592}        & \textbf{2.081/0.645}        & \textbf{2.145/0.653}        & 2.01/0.62    & \textbf{2.01/0.62} &\\

Hero~\cite{burnett2021radar} &~\cite{burnett2021radar} & $0.2628$ & 1.77/0.62          & \textbf{1.75/0.59}        & 2.04/0.73        & 1.83/0.61        & 2.20/0.77        & 2.14/0.71        & 2.01/0.61        & 1.97/0.65        & 
1.96/0.66$^*$    & 
N/A\\
\ac{TITLE} (ours) &  & $0.043$ & \textbf{1.64/0.48}          & 1.86/0.52        & \textbf{1.66/0.48}        & \textbf{1.71/0.49}        & \textbf{1.75/0.51}        & \textbf{1.65/0.48}        & \textbf{1.99/0.53}        & \textbf{1.79/0.5}        & 
1.76/0.50 & \textbf{1.76/0.50} 
\end{tabular}
  \end{adjustbox}

\caption{Evaluation on 8 sequences with different methods and sensor modalities on the Oxford Radar RobotCar dataset~\cite{RadarRobotCarDatasetICRA2020}.  Results are given in (\% translation error / deg/$100$~m). Note the difference between columns "Mean" and "Mean SCV". In "Mean" column, methods marked $^*$ cannot be compared directly as these are trained and evaluated on the same spatial location. The most relevant number for comparison is instead "Mean SCV" which ensures that test and training data are not correlated by using spatial cross validation. 
}
\label{tab:results}
\vspace{-0.2cm}
\end{table*}


%Since neither of ~\cite{8460687,barnes_masking_2020} has an opensource implementation and the results reported in their papers only include mean errors, there is no detailed errors for each ssequence. 


%WARNING WARNING - EXAMPLE TEXT OF EVALUATION DIRECTLY COPIED FROM OTHER PAPER

%The quantitative evaluation is to understand the pose estimation accuracy of the proposed RadarSLAM system. We follow the popular KITTI odometry evaluation criteria, i.e., computing the mean translation and rotation errors from length 100 to 800 meters with a 100m increment. Stateof-the-art odometry and SLAM algorithms using different sensors are also compared. 


%The Oxford Radar RobotCar Dataset is used for the quantitative evaluation as it is an open large-scale radar dataset easy for benchmarking. It includes 32 sequences of radar data collected while traversing a same route in Oxford with ground truth poses. The radar data is captured by a Navtech CTS350-X, a Frequency Modulated Continuous Wave (FMCW) scanning radar. It is configured to return 3768 power readings at a resolution of 4.32cm across 400 azimuths and operates at the frequency of 4Hz (with maximum range of 163m)

%\begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
% \hline
% Country Name     or Area Name& ISO ALPHA 2 Code &ISO ALPHA 3 Code&ISO numeric %Code\\
% \hline
% Afghanistan   & AF    &AFG&   004\\
% Aland Islands&   AX  & ALA   &248\\
% Albania &AL & ALB&  008\\
% Algeria    &DZ & DZA&  012\\
% American Samoa&   AS  & ASM&016\\
% Andorra& AD  & AND   &020\\
% Angola& AO  & AGO&024\\
% \hline
%\end{tabular}
\subsection{Qualitative evaluation}
In order to assess the generality of the method, additional non-urban  data was collected. We perform a qualitative evaluation of radar odometry in two different industrial scenarios using 
%the Navtech radar model 
another Navtech \ac{FMCW} radar model,
CIR154XH. 
For these datasets, the sensor was configured with range resolution $\gamma=17.5$cm, with $400$ azimuth bins. Ground truth positioning is missing in these datasets. However, we estimate the error between the first and final scan by comparing the offset between duplicated landmarks in the map which gives a rough indication of odometry drift.
%\todo{Martin: don't forget to include the numbers in the text (even if they are just a "rough indication")}

\subsubsection{Evaluation in semi-structured outdoor environment -- Volvo CE}
\label{sec:volvo_eval}

The first dataset was collected from a test track for wheel loaders and dump trucks in a partly forest environment driven at an approximate speed of $10$km/h. The track consists mainly of gravel roads at various slopes and the radar sensor was mounted on the driver cabin of a Volvo wheel loader (see Fig.~\ref{fig:volvo_test_track_and_vehicle}). The larger loop in Fig.~\ref{fig:volvo_test_track_and_vehicle} is $1150$ meters long. After completing the larger gravel-road loop, two smaller loops were traversed on uneven paths inside the forest reaching a total trajectory length of $1605$ meters. We expect this highly cluttered environment to be challenging for \ac{TITLE} that attempts to reconstruct and utilize surface normals.


%%%%%%%%%%%% PREVIOUS %%%%%%%%%%%%%
%To achieve best performance, the minimum power return was increased to $z_{min}=85$. This can be related to the change of sensor model and range configuration from the previous dataset, or related to the characteristics of the environment. Fig.~\ref{fig:volvo_after_revisit} depicts the trajectory just before revisiting the start of the loop, and the full trajectory with $s=3$ keyframes, compared to a single submap keyframe. In line with our previous results, increasing the amount of submap keyframes reduces the drift over the large and small loops. This can be seen by the relatively higher blur in fig.~\ref{fig:volvo_full_nosubmap} compared to fig.~\ref{fig:volvo_full_submap}. We believe this is because additionally constraining the registration reduces pose estimate noise but also due to the uneven driving conditions, especially in the forest, where the radar is not fully planar.



 %\begin{figure}
 % \begin{center}
  %  \subfloat[Vehicle test track. A wheel loader with radar starts inside the white tent (right) and is driven large loop on a gravel road and then in two smaller loops on an uneven path in the forest. The full trajectory is visualized in fig.~\ref{fig:volvo_full_submap}.]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.99\hsize]{figures/volvo_qualitative/google_earth_volvo_downsampled.jpg}\label{fig:volvo_map}}\hfill \\
   %     \subfloat[Driving on a narrow uneven path in the forest. ]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.49\hsize]{figures/volvo_qualitative/loader_forest_downsampled.jpg}\label{fig:volvo_forest}}\hfill
    %    \subfloat[Driving on gravel road uphill.]{\includegraphics[trim={0.0cm 0cm 0   cm 0cm},clip,width=0.49\hsize]{figures/volvo_qualitative/loader_road_downsampled.jpg}\label{fig:volvo_road}}\hfill \\
    %\vspace{-0.2cm}
 %   \caption{\label{fig:volvo_test_track_and_vehicle}}
 % \end{center}
  %\end{figure} %\vspace{-0.3cm}
%\begin{figure}
%  \begin{center}
%    \subfloat[Estimated path (red) and map (black) before revisit. Grid size ($10\times 10$m).  ]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.89\hsize]{figures/volvo_qualitative/1.png}\label{fig:volvo_before_revist}}\hfill 
%    \\
%    \subfloat[Full estimated trajectory ($1650$m) with using 3 submap key-frames. The Map is blurred at the revisited regions of the large loop due to odometry drift but fairly sharp around the small loop. We estimate the final position error to $2.5$m ($0.2\%$).]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.89\hsize]{figures/volvo_qualitative/5.png}\label{fig:volvo_full_submap}}\hfill \\
%    \subfloat[Full estimated trajectory with a single key-frame yeld rougly ($0.4\%$ error). The map is more additionally distorted, now also around the small loop.]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.89\hsize]{figures/volvo_qualitative/nosubmap/no_submap_full.png}\label{fig:volvo_full_nosubmap}}\hfill %\\
 %   \caption{\label{fig:volvo_after_revisit}}
%  \end{center}
  %\vspace{-0.3cm}
%\end{figure}

%%%%%%%%%%%% Updated %%%%%%%%%%%%%
The estimated odometry and a corresponding map, obtained without changing parameters from the urban dataset, is depicted in Fig.~\ref{fig:volvo_oxford_parameters}. The maximum translation error is $15$~m ($1.3$\%) over the large loop. We notice that $\zmin=55$ is too low in combination with the sensor model and cluttered forest environment, however, \textit{k-strongest filtering} limits the amount of noise included in the filtered point cloud. We also note that motion compensation can have a negative impact in this dataset. For that reason, we made an attempt to improve the odometry by increasing the power threshold $\zmin=85$, by switching off motion compensation, and by increasing surface point density to $f=3$. These parameters reduced the estimated error to $2.5$~m ($0.2)$\% as depicted in Fig.~\ref{fig:volvo_full_submap}. For comparison, we plot the odometry with updated parameters but with a single submap keyframe $s=1$, this increases the error to $5~$m ($0.4$\%) as seen in Fig.~\ref{fig:volvo_full_nosubmap}.
%As depicted in in Fig.~\ref{fig:volvo_full_submap} with $s=3$ submap keyframes and in fig.~\ref{fig:volvo_full_nosubmap} with $s=1$ keyframes
In line with our previous results, increasing the number of submap keyframes reduces the drift. This can be seen by the relative increase in map blur in Fig.~\ref{fig:volvo_full_nosubmap} ($s = 1$) compared to Fig.~\ref{fig:volvo_full_submap} ($s = 3$). We believe this is because additionally constraining the registration reduces pose estimate noise and increases robustness due to uneven driving conditions, especially in the forest.



 \begin{figure} 
 \vspace{0.2cm}
  \begin{center}
    \subfloat[Vehicle test track. A wheel loader with radar starts inside the white tent (right) and is driven in a large loop on a gravel road and then in two smaller loops on an uneven path in the forest. The full driven trajectory (seen in red) is imported from Fig.~\ref{fig:volvo_full_submap}.
    The locations of the photos in figure (b) and (c) are indicated along the trajectory.
    ]%
    {\begin{tikzpicture}
    \node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[trim={0.0cm 0cm 0cm 2cm},clip,width=0.99\hsize]{figures/Volvo/overlayed_eskilstuna_downsampeld.jpg}};
    \node[white!70!white] at(1.6,5.7) {(\textbf{b})};
    \node[white!70!white] at(3.5,5.3) {(\textbf{c})};
    \end{tikzpicture}}
    %\vspace{-1cm}
    %{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,width=0.99\hsize]{figures/volvo_qualitative/overlayed_eskilstuna_downsampeld.jpg}\label{fig:volvo_map}}\hfill 
    \\
        \subfloat[Driving on a narrow uneven path in the forest. ]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,height=43mm]{figures/Volvo/loader_forest_downsampled.jpg}\label{fig:volvo_forest}}\hfill
        \subfloat[Driving on a gravel road uphill.]{\includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,height=43mm]{figures/Volvo/loader_road_downsampled.jpg}\label{fig:volvo_road}}\hfill \\
    
    \caption{Overview of semi-structured VolvoCE dataset.\label{fig:volvo_test_track_and_vehicle}}
  \end{center}
  \vspace{-0.8cm}
  \end{figure} %\vspace{-0.3cm}
\begin{figure}
\vspace{0.2cm}
  \begin{center}
    \subfloat[Full estimated trajectory (red) and map (black), obtained reusing parameters tuned for the Oxford urban dataset. The maximum estimated large loop error is $15$~m ($1.3$\%). Grid size ($10\times 10$)~m.  ]{\includegraphics[trim={0.0cm 0cm 0cm 0.5cm},clip,width=0.89\hsize]{figures/Volvo/same_parameters.png}\label{fig:volvo_oxford_parameters}}\hfill 
    \\
    \subfloat[Odometry improved by tailoring parameters to the VolvoCE dataset (motion compensation switched off, $\zmin=85$, $f=3$). The Map is blurred around revisited regions of the large loop due to odometry drift but fairly sharp around the small loop. We estimate the maximum large loop position error to be $2.5$~m ($0.2\%$).]{\includegraphics[trim={0.0cm 0cm 0cm 1cm},clip,width=0.89\hsize]{figures/Volvo/5.png}\label{fig:volvo_full_submap}}\hfill \\
    \subfloat[Full estimated trajectory with a single key-frame. The maximum large loop error is estimated to be $5$~m ($0.4\%$ error). The map around the large and small loop is more distorted compared to \ref{fig:volvo_full_submap}.]{\includegraphics[trim={0.0cm 0cm 0cm 1cm},clip,width=0.89\hsize]{figures/Volvo/nosubmap/no_submap_full.png}\label{fig:volvo_full_nosubmap}}\hfill \\
    \caption{Qualitative evaluation in VolvoCE dataset using various parameters.% with standard parameters (a), improved parameters (b), and improved parameters with a single submap keyframe (c).
    \label{fig:volvo_after_revisit}}
  \end{center}
  \vspace{-0.5cm}
\end{figure}



\subsubsection{Evaluation in mine -- Kvarntorp}
\label{sec:kvarntorp_eval}
In the final experiment we mounted the Navtech CIR154XH radar on a car and drove through a $1235$-m long loop in an underground mine, at an approximate speed of $10$~km/h. The environment is depicted in Fig.~\ref{fig:kvarntorp_example}. The solid walls are highly radar-reflective and the interaction between radar, mountain walls and the car gives rise to a large amount of strong multi-path reflections. In contrast to the other evaluated datasets, the tunnels in parts of this environment have limited amount of features that can constrain the registration in the longitudinal direction. 

Reusing the parameters tuned for Oxford dataset, we found that our method was able to reconstruct an accurate map of the environment with an estimated final position error of $15$~m ($1.2)$\% translation error. There are no visible errors in the passages between the top and bottom aisles in Fig.~\ref{fig:kvarntorp_example}, which is an indication that the method works well, even in a feature poor environment.




 %\begin{figure}
 % \begin{center}
 %   {\includegraphics[trim={3.0cm 0cm 3cm 0cm},clip,width=0.99\hsize,angle=0]{figures/kvarntorp/1_normals.png}\label{fig:kvarntorp_odometry}}
 %   \caption{Estimated odometry (red) and map (black), grid cell size $10$m $\times 10$m. We estimate the final translation error to $10$m ($0.8\%)$ }\label{fig:kvarntorp_odometry}
 % \end{center}
 % \vspace{-0.3cm}
%\end{figure} 
%\subfloat[Map created the Kvarntorp mine using our proposed radar odometry combined with an appearance based loop closure (not presented here).  ]{\includegraphics[trim={8.0cm 0cm 7cm 1cm},clip,width=0.49\hsize,angle=0]{figures/kvarntorp/full_loopclosure.png}\label{fig:kvarntorp_map}}\hfill

==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/Introduction.tex <==
Estimating odometry in large-scale GNSS-denied environments is an essential part in any robust autonomous driving or robotics system. Popular systems are based on lidar~\cite{todor_ndt,gicp,loam,behley2018rss}, vision~\cite{zhu2017image,Buczko_vis_odom,6906584}, introceptive sensors such as IMU or wheel odometry, or a combination of various sensors~\cite{7139486,8202318,narula_all-weather_2020}.
%Internal sensors: greatly suffers from drift.

Lidar is an accurate and fast long-range sensor but struggles to perceive the environment in presence of dust or in harsh weather~\cite{acarballo2020libre}. Vision is moderately accurate and inexpensive but operates at shorter range and is sensitive to illumination changes or weather conditions. In contrast, radar is a long-range sensing modality that operates well in all weather conditions and is hardly affected by smoke and dust. As radars have recently become compact enough for autonomous systems, it is desired to utilize their excellent properties for robust localization.
%These are desired sensor properties for 
%As these senors have recently become practical %localization and are therefore promising
\begin{figure}
  %\begin{center}
  %\subfloat[]
      {\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.99\hsize,angle=0]{figures/Kvarntorp/oxford_parameters_filter.jpg}\label{fig:kvarntorp_odometry}}\hfill\\
    \includegraphics[trim={0.0cm 0cm 0cm 0cm},clip,height=0.29\hsize,angle=0]{figures/Kvarntorp/car_downsampled.jpg}\label{fig:kvarntorp_vehicle}
      \includegraphics[trim={0.0cm 1cm 0cm 2cm},clip,height=0.29\hsize,angle=0]{figures/Kvarntorp/kvarntorp2.jpg}\label{fig:kvarntorp_mine}
    \caption{
    Example output using the proposed method. Incremental odometry estimated from a roof-mounted radar in an underground mine using the proposed method with no additional sensor. Parameters are tuned for a different sensor in an urban environment but generalize well. The accumulated error is roughly $15$m over a distance of $1235$m driving ($1.2$\%).
    Our system is demonstrated at: \url{https://youtu.be/np-ceNrAcNY}.
    %Odometry estimated in an underground mine using only a roof-mounted radar with the proposed method.
    }\label{fig:kvarntorp_example}
 % \end{center}
  \vspace{-0.3cm}
\end{figure}

State-of-the-art radar odometry systems put great effort into overcoming sensor-specific challenges such as speckle noise, ghost objects and false positives %This is typically addressed 
using deep learning methods to remove noise~\cite{barnes_masking_2020}, predict keypoints~\cite{barnes_under_2020,burnett2021radar}, and through robust data association algorithms~\cite{hong2021radar,8460687,8793990}. Scan matching is then based on sparse and efficient keypoints~\cite{barnes_under_2020,hong2021radar,8460687,8793990} or dense radar images~\cite{barnes_masking_2020,9197231}.% We note that there is currently no sparse radar matching method that make use of surface models, which has been proven successful in other sensor modalities.

%Existing methods based on Deep convolutional neural networks~\cite{barnes_under_2020,barnes_masking_2020} require an extensive amount of training data (from over 200~km of driving), with ground-truth odometry. Additionally, their odometry quality deteriorates when running in locations or environments types not included in the training-set~\cite{barnes_masking_2020}. 
 
%For these reasons, we want to explore learning-free approaches based on surface models that can bring efficient and accurate formulations to the radar odometry problem, and generalize across environments.
While learning-based methods perform well on locations included in the training set, they provide limited generalization and, accordingly, their accuracy deteriorates at previously unseen locations~\cite{barnes_masking_2020} (despite being trained with data acquired from over 200~km of driving)~\cite{barnes_under_2020,barnes_masking_2020}.
Previous sparse methodshave
%\todo{Some problems of making a coherent argument here}

%We note that there is currently no sparse radar matching method that makes use of surface models, which has been proven successful in other sensor modalities.

%neural networks~\cite{barnes_under_2020,barnes_masking_2020} require an extensive amount of training data (from over 200~km of driving), with ground-truth odometry. Additionally, their odometry quality deteriorates when running in locations or environments types not included in the training-set~\cite{barnes_masking_2020}. 
 
We present \ac{TITLE}, a learning free method for efficient and accurate large-scale odometry estimation.
\ac{TITLE} filter radar data that creates a sparse representation in which the environment is modeled as a set of oriented surface points as depicted in Fig.~\ref{fig:k_strong_normals}. By keeping only the $k$ strongest power returns per measurement azimuth above the expected noise level, %at the corresponding range-bin, 
a conservative but sufficient set of points can be maintained while removing most radar noise. The filtered radar returns can be used to create a sparse set of surface points and normals that models the underlying geometry of important surface features. Scan registration is efficiently carried out by minimizing a point-to-line metric between correspondences, using a Huber loss function to achieve robustness to outliers.

The central contribution of this paper is an efficient, accurate and robust method tailored for spinning \ac{FMCW} radar in large-scale environments, improving state-of-the-art accuracy on a public benchmark data set. Our results show that \ac{TITLE} method performs well in widely different environments (urban, forest, tunnel/mine) and can be used with different sensor models without changing a single parameter. It requires no training and runs on a single-core laptop CPU at $55$~Hz.


%We make the following claims


%allow efficient scan representation for accurate and fast scan registration. By using a simple heuristic that keeps the strongest returns per azimuth, only points on the first 


%\begin{figure}
%\centering
%\begin{subfigure}%{\textwidth}
%  \centering
%  \includegraphics[width=\linewidth,trim={10cm 2cm 10cm 5cm},clip]{figures/sweep/1}
%  \caption{Raw radar sweep impaired by speckle noise and reflections.}
%  \label{fig:sub1}
%\end{subfigure}%
%\begin{subfigure}%{\textwidth}
%  \centering
%  \includegraphics[width=\linewidth,trim={10cm 2cm 10cm 5cm},clip]{figures/sweep/4}
%  \caption{Processed radar data(black points) with surface normals (red arrows).}
%  \label{fig:sub2}
%\end{subfigure}
%\caption{\label{fig:scan_normals}A figure with two subfigures}\textbf{}
%\end{figure}

 %\begin{figure}
 % \begin{center}
 %   \subfloat[Raw radar sweep impaired by speckle noise and reflections.]{\includegraphics[width=\hsize,trim={10cm 2cm 10cm 5cm},clip]{figures/sweep/1}\label{fig:sub1}}\hfill
    %\subfloat[Processed radar data (black points) with estimated surface normals (red arrows). Efficiently modeling surfaces is possible by keeping only a minimum amount of points. ]{\includegraphics[width=\hsize,trim={10cm 2cm 10cm 5cm},clip]{figures/sweep/4}\label{fig:sub2}}\hfill
    %\caption{\label{fig:scan_normals}A figure with two subfigures}
  %\end{center}
  %\vspace{-0.3cm}
%   \end{figure}

==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/backup/introduction_backuo.tex <==
%Determining if point clouds are correctly aligned is essential to enable robust mobile robotics. Applications such as mapping, scene understanding and sensor calibration are prone to miss alignment of point clouds and requires capability to asses reliability of scan alignment used in the process to avoid devastating failures. Alignment error occurs due to uncompensated motion distortion or wrong convergence in the scan registration.  Our system: ``CorAl'' can detect both these type of errors in real-time, even with small alignment errors. 
%Our method  is well grounded in information theory which and we provide an intuitive formulation of the problem. CorAl measures the difference between the entropy of the merged and separate point clouds and can be used to detect miss alignment. For aligned point clouds, the merged cloud and separate point clouds are similarly blured which provides a measure close to zero. In contrast, merged misaligned point clouds tend to ``blur'' the scene which can be observed by the increase in entropy. The separate point clouds are used to discount for the entropy of the scene. Consequently, the measure provides an absolute understanding of the alignment reliability.\\\\


In order to create safe and efficient mobile robots, introspective capabilities are required to assess and recover from perception failures. Various perception tasks, including localization~\cite{zhang_loam_2014,adolfsson_submap_2019}, scene understanding and sensor calibration~\cite{della_corte_unified_2019}, rely on point cloud registration. However, registration may provide incorrect estimates due to wrong convergence, uncompensated motion distortion, sensor noise or lack of features~\cite{andreasson_incorporating_2017}, potentially causing a system failure or hazard. Consequently, it is essential that the quality of registration is assessed, and unsuccessful attempts are rejected or re-estimated.

In the past, various methods have been proposed to assess the alignment quality of point cloud pairs. One category of methods attempts to provide an uncertainty estimate between point clouds~\cite{David_Landry,bengtsson_robot_2003, nieto_scan-slam_2006,prakhya_closed-form_2015}. However, these methods rely on the assumption that the registration has reached a global maximum -- which may be invalid --  and cannot be used to assess absolute alignment quality.

%perhaps more expli
More recently, Almqvist et al. presented a learning approach to detect misaligned point clouds ~\cite{Almqvist}. A strong classifier was trained based on weaker classifiers derived from common point cloud measures~\cite{rusinkiewicz-2001-fasticp,biber_normal_2003,magnusson-2009-phd,chandran-ramesh_assessing_2007,makadia-2006-fully,silva-2005-ga}.
%~\cite{akai_misalignment_2019,biber_normal_2003, stoyanov_comparative_2013, magnusson-2009-phd}. 
The classifiers were evaluated on two outdoor data sets, and although the combined classifier, as well as some of the individual ones, reach almost 90\,\% classification accuracy for the hardest cases on each data set individually, accuracy dropped to around 80\,\% when cross-evaluating between the data sets.
%The authors reported significantly reduced classification accuracy for all evaluated classifiers when applied to new environments. A key reason for the lack of robustness to environmental changes is that current classifiers do not account for the appearance of the environment and rely heavily on parameter tuning.\\

%Alqvist writes that ``we hope that more specific classifiers will be investigated''.
%Work by  Chandran-Ramesh and Paul Newman ~\cite{chandran-ramesh_assessing_2007} later adopted to pointcloud-pairs by almqvist
%akai_misalignment_2019 detect localization error.
%ICP COVARIANCE Monte Carlo: bengtsson_robot_2003
% closed form ~\cite{nieto_scan-slam_2006}.
% closed formprakhya_closed-form_2015
%useful for pose-graph optimization.
In this paper, we propose ``CorAl'': an accurate and fast  alignment measure and binary classifier for point cloud pairs to bridge the gap in classification performance when the method is applied in new unseen environments without retraining.

% both these type of errors in real-time, even with small alignment errors. CorAl 
Our method is well grounded in information theory and gives an intuitive formulation to the alignment quality problem. CorAl measures the difference between the entropy of the merged and separate point clouds. For well-aligned point clouds, the merged cloud and separate point clouds
have similar entropy %are similarly blured 
and provide a measure close to zero. In contrast, misaligned point clouds tend to ``blur'' the scene which can be observed by an increase in entropy. The separate point clouds are used to discount for the entropy inherent in  the scene. Consequently, the measure provides an absolute understanding of the alignment quality. 





%This work is related to large-scale localization and mapping. THere are multiple essential parts in such system and depending on the application requirements they techniques may vary significantly. Many localization problems are related to finding the alignment between point clouds. If the relative alignment is known, the motion or the location of the robot has been determined. Most systems find the alignment by making assumptions on the quality and relative alignment of point clouds and then deploy well established methods from mathematics to solve the alignment. If any of these assumptions are violated, the localization is likely to fail. For example. Most lidar odometry systems uses the motion of the wheel of the robot to compensate for distortion in the data. based on this correction, local registration methods are used to find the relative alignment. This scenario is likely to introduce two different errors, at least to some extent. The first error is that the motion compensation is inaccurate due to slippage, unsyncronized sensors or noise. This causes the data be inaccurate. The second problem depend on that local registration methods have a limited convergence basin. The registration can fail if the initial alignment is not sufficiently close to the true solution. If the localization algorithms is able to detect occurance of such problems, it can likely also be build to manage and recover from them. Thus making more robust localization systems for robots.

The contribution of this paper is an intuitive and simple measure of the absolute alignment quality between pairs of point clouds based on a relative change in scene entropy. We demonstrate how to use this quality measure to learn to detect misaligned point clouds and how to utilize our tool for manual inspection of alignment quality.
We provide an open source ROS/C++ implementation\footnote{https://github.com/dan11003/CorAl-ScanAlignmentClassification} and make our evaluation available to the community. 

We make the following claims: (i) Our proposed measure provides an absolute understanding of alignment quality by accounting for the expected scene entropy. 
(ii) Our method is highly accurate in %specific environments, 
a wide range of environments and %can even improve adaptation to new unseen environments compared to state-of-the-art alignment classification.
generalizes well to new environments without retraining.





%Fig.~\ref{fig:example_1} 


==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/backup/related_work_backup.tex <==
 
Various methods have been used to assess alignment quality. Traditional methods calculate the root mean squared (RMS) point-to-point error, which also is the function that
is minimised by iterative closest point (ICP) registration~\cite{ICP}, or a point-to-distribution~\cite{ndtbiber} distance.
%The minimization is typically stopped when a local minima is found or a maximum number of iterations are reached.
As reported in Almqvist et al.~\cite{Almqvist}, the absolute level of score is sensitive to method parameters, environment and sensing noise. Consequently, they are  are poorly suited for global alignment classification. 

A family of methods attempts to estimate the alignment uncertainty between point cloud pairs. 
Some use Monte Carlo strategies to estimate uncertainty by sampling registrations in a region. This exhaustive search is however unpractical in mobile robotics.
Other attempt to estimate uncertainty in closed form using the Hessian, representing the steepness of the alignment score function around a local minima. These methods assumes correct alignment as they are fundamentally limited by the traditional alignment scores. Consequently, the uncertainty estimation and cannot give an absolute alignment quality. 

Almqvist et al.~\cite{Almqvist} extensively explored building classifiers based on the traditional RMS and Point-to-distribution (P2D) scores. 
The authors also derived a classifier based on Chandran-Ramesh and Newman~\cite{chandran-ramesh_assessing_2007}, which attempts to find suspicious regions in the map, counting planar intersections. The authors proposed AdaBoosting for fusing and improving the individual classifiers. While this did not have a major impact on the classification accuracy, their method reduced parameter sensitivity. %When evaluating the learned classifiers to new environments, RMS and NDT-P2D scored around 50\% accuracy. %While modifying NDT-P2D showed improved performance.
While RMS and L2 classifiers performed on par with random when transferred into new environments without adjusting parameters.
We notice that this limitation inherits from the traditional distance measures.

Liao et al. \cite{fuzzybnb} recently proposed a global registration method representing point clouds as fuzzy sets. The method first attempts to find a consistent clustering by centering clusters at representative locations. A measure that compares the similarity of points distributions around cluster centers is then used to provide a quality assessment in the absence of ground truth. 
Unlike other global registration methods, the quality assessment is used as a stop criteria to end the global search when a coarse alignment is reached. Afterwards, fine tuning is applied to refine this coarse solution and obtain a precise alignment. 
This quality assessment is not sensitive to small misalignment. Accordingly, we categorize this work as coarse alignment quality assessment. In this work we're interested in fine alignment quality assessment.
%%The argument of this quality assessment builds on the robustness of the fuzzy center points. When wil this perform and when will it not?
%As the clustering comes with a high complexity, the method is intractable without downs
Additionally, the method requires at least 50\% overlap between the point clouds which may not be possible in mobile robotic applications. 
Our methods does not require a minimum overlap by operating principle, however we consider point clouds with less than 10\% overlap to provide insufficient evidence to determine alignment quality.\\
%WHy not calculate standard error to determine if there exists evidence for overlap????? 
To the best of our knowledge, there is no method for binary classification of point clouds alignment that performs accurate in real-time and adapts well to new environments.\\

The rest of the paper is structured as follows:
In section \ref{sec:method} we describe our alignment measure and how to train it for binary classification. In section \ref{sec:eval} we propose a benchmark test for further research in the area and evaluate our method on publicly available data.
%https://github.com/zgojcic/3DSmoothNet deep learning high recall
%  Chandran-Ramesh and Paul Newman 

%Introduction
%relative alignment  - local registration
% icp - rms
% ndt - l2 distance
% limited convergence basin - unsuitable for quality assesment
% Broad convergence basin Efficient Global Optimization

%


%Global typically costly, for offline.

%ICP measure%A method for registration of 3-D shapes
%Alqvist et al. \cite{Almqvist} uses AdaBoost to improve a set of weak classifiers.

%Similar covariance estimation}

==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/figures/Parameters/figure_k_points.tex <==
\begin{tikzpicture}
	\begin{axis}
	[
		width   = 0.9\columnwidth,
		height  = 0.6\columnwidth,
		xmin		= 55,
		xmax		= 135,
		ymin		= 0.1,
		%ymax		= 0.05,
		%ytick	= {0, 0.25, ..., 1},
		xlabel  = {range $[m]$},
		ylabel  = {scaled power},
		ylabel near ticks,
		%	ylabel shift			= 2,
%		ymode = log,
		legend style={
			at={(0.5,1.5)},
			anchor= north,
			fill = none,
			draw=none,
			},
		legend columns			= 2,
	]
	\addplot
	[
		white!70!black,
		thick,
		%only marks,
%		mark size	= 0.02cm,
%		mark		= *,
	]
	table
	[
		x   = range,
		y   = beam,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{measurements};
	%%%
%	\addplot
%	[
%		white!50!black,
%		thick,
%		dashed,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
%	]
%	table
%	[
%		x   = range,
%		y   = thr_k,
%	]
%		{Datasets/export_figure_threshold.txt};
%		\addlegendentry{$k=12$ threshold};
	%%%
	\addplot
	[
		white!25!black,
%		thick,
		solid,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
	]
	table
	[
		x   = range,
		y   = thr_cfar,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{CFAR threshold};
	%%%
	\addplot
	[
	white!25!black,
	thick,
	dotted,
	%only marks,
	%		mark size	= 0.02cm,
	%		mark			= *,
	]
	table
	[
	x   = range,
	y   = thr_noise,
	]
	{Datasets/export_figure_threshold.txt};
	\addlegendentry{$\zmin$ threshold};
%	
	\addplot
	[
	white!5!red,
%	thick,
%	dotted,
	only marks,
	mark size	= 0.08cm,
	mark		= o,
	]
	table
	[
	x   = range,
	y   = k_12,
	]
	{Datasets/export_figure_threshold.txt};
	\addlegendentry{$k=12$ detection};
	\addplot
	[
	white!5!blue,
	%	thick,
	%	dotted,
	only marks,
	mark size	= 0.06cm,
	mark		= +,
	]
	table
	[
	x   = range,
	y   = cfar,
	]
	{Datasets/export_figure_threshold.txt};
	\addlegendentry{CFAR detection};	
	\end{axis}
\end{tikzpicture}


==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/figures/Parameters/figure_k_threshold.tex <==
\begin{tikzpicture}
	\begin{axis}
	[
		width   = 0.95\columnwidth,
		height  = 0.6\columnwidth,
		xmin		= 0,
		xmax		= 90,
		ymin		= 2,
		%ymax		= 0.05,
		%ytick	= {0, 0.25, ..., 1},
		xlabel  = {range $[m]$},
		ylabel  = {scaled power},
		ylabel near ticks,
		ymode = log,
		%	ylabel shift			= 2,
		legend style={
		at={(0.5,1.4)},
		anchor= north,
		fill = none,
		draw=none},
		legend columns			= 2,
	]
	\addplot
	[
		white!70!black,
		very thick,
		%only marks,
%		mark size	= 0.02cm,
%		mark			= *,
	]
	table
	[
		x   = range,
		y   = beam,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{measurements};
	%%%
	\addplot
	[
		white!75!black,
		thick,
		dotted,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
	]
	table
	[
		x   = range,
		y   = thr_k,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{strongest $k$ threshold};
	%%%
	\addplot
	[
		white!25!black,
		thick,
		solid,
		%only marks,
		%		mark size	= 0.02cm,
		%		mark			= *,
	]
	table
	[
		x   = range,
		y   = thr_cfar,
	]
		{Datasets/export_figure_threshold.txt};
		\addlegendentry{CFAR threshold};
	%%%
	\addplot
	[
	white!25!black,
	thick,
	dotted,
	%only marks,
	%		mark size	= 0.02cm,
	%		mark			= *,
	]
	table
	[
	x   = range,
	y   = thr_noise,
	]
	{Datasets/export_figure_threshold.txt};
	\addlegendentry{noise threshold};
	\end{axis}
\end{tikzpicture}


==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/figures/Parameters/figure_submap_key_frame.tex <==
\begin{tikzpicture}

\pgfplotsset{width=7.5cm,compat=1.12}
  \pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
	width   = 0.7\columnwidth,
	height  = 0.45\columnwidth,  
	ymin		= 1.72,
	ymax		= 1.95,
	legend style={at={(0.5,0.95)},anchor= north},
    axis y line*=left,
    xlabel={number of submap keyframes},
    ylabel={translation error [$\%$]},
  ]
    \addplot[mark=*,white!50!red,very thick]
      coordinates{
    (1.0000, 1.9100)
    (2.0000, 1.8100)
    (3.0000, 1.7300)
    (4.0000, 1.7200)
        % more points
      }; \label{plot_1_y1}

    \end{axis}

    \begin{axis}[
		width   = 0.7\columnwidth,
		height  = 0.45\columnwidth,
	ymin		= 15,
	ymax		= 65,
	legend style={at={(0.5,0.95)},anchor= north},
    axis y line*=right,
    axis x line=none,
    ylabel={computation time [ms]},
    ]

    \addplot[mark=x,blue!75!black,thin]
      coordinates{
    (1, 19.0795)
    (2, 28.6807)
    (3, 40.5221)
    (4, 53.5934)
        % more points
      }; \label{plot_1_y2}
    
    \addlegendimage{/pgfplots/refstyle=plot_1_y1}\addlegendentry{computation time}
    \addlegendimage{/pgfplots/refstyle=plot_1_y2}\addlegendentry{translation error}
  \end{axis}

\end{tikzpicture}

==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/figures/Parameters/figure_translation_rotation_error.tex <==
\begin{tikzpicture}
\pgfplotsset{width=7.5cm,compat=1.12}
  \pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
  	width   = 0.7\columnwidth,
	height  = 0.45\columnwidth,
	ymin		= 1,
	ymax		= 8,
	legend style={at={(0.5,0.95)},anchor= north},
    axis y line*=left,
    xlabel={$k$ strongest return},
    ylabel={translation error [$\%$]},
  ]
    \addplot[mark=*,white!50!red,very thick]
      coordinates{
    (1.0000,    4.3300)
    (3.0000,    2.1000)
    (12.0000,    1.8100)
    (25.0000,   1.7100)
    (30.0000,    1.6800)
    (35.0000,   1.6500)
    (40.0000,    7.6000)
    (50.0000,   41.6100)
        % more points
      }; \label{plot_1_y1}

    \end{axis}

    \begin{axis}[
	width   = 0.7\columnwidth,
	height  = 0.45\columnwidth,
	ymin		= 0.4,
	ymax		= 1.3,
	legend style={at={(0.5,0.95)},anchor= north},
    axis y line*=right,
    axis x line=none,
    ylabel={rotation error $\deg$/100m},
    ]

    \addplot[mark=x,blue!75!black,thin]
      coordinates{
    (1.0000,  1.1600)
    (3.0000,  0.6900)
    (12.0000, 0.5600)
    (25.0000, 0.5300)
    (30.0000, 0.5200)
    (35.0000, 0.5100)
    (40.0000, 1.0800)
    (50.0000, 4.1900)
        
        % more points
      }; \label{plot_1_y2}
    
    \addlegendimage{/pgfplots/refstyle=plot_1_y1}\addlegendentry{translation error}
    \addlegendimage{/pgfplots/refstyle=plot_1_y2}\addlegendentry{rotation error}
  \end{axis}

\end{tikzpicture}

==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/method.tex <==
\section{Spinning radar sensing}
\label{sec:method}
Our method \ac{TITLE} is tailored for, but not specific to, a spinning \ac{FMCW} radar without Doppler information. 
At the end of each full $360^\circ$ sweep, the sensor outputs a full power reading  $Z_{m \times n}$ in polar form, where $m$ is the amount of azimuths per sweep and $n$ is the amount of range bins per azimuth. Each azimuth and range bin $(a,d)$ in $Z_{m \times n}$ stores a power return and can be converted from polar to Cartesian space as seen in Fig.~\ref{fig:polar_2_cart} using Eq.~\eqref{eq:cartesian}.
\begin{equation}
\label{eq:cartesian}
    \mathbf{p} = \begin{bmatrix} d \gamma \text{cos}\left(\theta\right) \\ 
    d \gamma \text{sin}\left(\theta\right)
\end{bmatrix},
\end{equation}
where $\theta=2\pi a/m$ and $\gamma$ is the range resolution set to $4.38$cm or $17.5$cm in our experiments.
\begin{figure}[H]
\vspace{0.2cm}
    \centering
\includegraphics[width=0.99\hsize]{figures/Radar_raw/polar_to_cartesian.png}
    \caption{Conversion between polar (left) $Z_{m\times n}$ and Cartesian (right) space. Each row and column in the polar image correspond to an angle and range $(a,d)$ in the Cartesian image.}
    \label{fig:polar_2_cart}
    \vspace{-0.2cm}
\end{figure}

\section{\ac{TITLE}}
%\todo{Martin: since this is the core of the contribution, some more detail is needed in this section. Most importantly, you need to describe/discuss $\zmin$}
We argue that it is hard to find stable keypoints from peaks per azimuth due to large beam width, and radar sensing artifacts. % For that reason
%We argue that filtering techniques that detect key-points from local peaks per azimuth can be sensitive to radar characteristics, such as large beam width and reflections, and this is indicated by our evaluation in Fig.~\ref{fig:k_eval}. This results in unstable key-points that are not representative for the underlying geometry and unsuitable for scan matching.
In \ac{TITLE}, we compute a scan representation in two steps. First, only the $k$ strongest returns with power exceeding $\zmin$ are selected at each azimuth and converted into Cartesian space. Second, oriented surface points are computed in Cartesian space by analyzing local point distributions at discrete intervals. This creates a sparse surface representation from the originally noisy radar data, which rejects artifacts such as multi-path reflections in favor of important landmarks.

\subsection{k-strongest filtering}
The typical behavior of \textit{$k$-strongest filtering} compared to the classical method CFAR can be seen in Fig.~\ref{fig:k_threshold}. Keeping only the $k$ strongest returns exceeding the power $\zmin$ reduces false positives at the expense of possibly missing landmarks with weaker returns. %This makes the method less sensitive to $z_{min}$.
%However as shown by our evaluation depicted in Fig.~\ref{fig:k_eval}, missing weaker landmarks has a negligible impact on localization accuracy. 
However as shown by our evaluation depicted in Fig.~\ref{fig:k_eval}, limiting the amount of returns has a small effect on odometry accuracy within a wide region.
This indicates that a conservative filtering technique is preferable for efficient radar odometry estimation.



%Filtering the radar data with a fixed or adaptive $z_{min}$ alone is generally hard to tune and is sensitive to surface material, incident angle and distance.
\subsection{Estimating oriented surface points}
Given the filtered point set $\bm{\mathcal{P}}_f$
we aim to model the underlying surfaces in the environment by a set of oriented points; i.e., surface points and normals $\{\bm{\mu}_i,\mathbf{n}_i\}$.
This is done by first downsampling the point cloud $\bm{\mathcal{P}}_f$ to $\bm{\mathcal{P}}_d$ using a grid with side length $r/f$~m, with 
$r$ the distance in which we expect to find sufficient amount of points to estimate the normal, and $f$ a re-sampling factor that adjusts the density of the final representation.
For each grid cell, only the centroid is kept.
%the points are downsampled by their point centroid. 


For each point in the downsampled point cloud $p_i \in \bm{\mathcal{P}}_d$, all neighbors of $p_i$ in $\bm{\mathcal{P}}_f$ within a radius $r$ (same $r$ as above), are used to estimate the point distribution by the sample mean and covariance $\{\bm{\mu}_i,\mathbf{\Sigma}_i\}$. 
Ill-defined distributions where the condition number $\kappa(\mathbf{\Sigma}_i)=\lambda_\mathrm{max}(\mathbf{\Sigma}_i)/\lambda_\mathrm{min}(\mathbf{\Sigma}_i) > 10^5$, or where distributions are estimated from less than $6$ points are discarded. This works as an additional filtering step that removes remaining false detections after \textit{k-strongest} filtering and ensures that surface points are estimated from a sufficient number of points and from multiple azimuths. The surface normal $\mathbf{n}_i$ is obtained from the smallest of the two eigenvectors of $\mathbf{\Sigma}_i$. The full scan representation $\bm{\mathcal{M}}$ is obtained by pairing all surface points and normals $\bm{\mathcal{M}} = \{\mathbf{\bm{\mu}}_i,\mathbf{n}_i\}$. An example of reconstructed surfaces after applying the \textit{$k$-strongest filter} in comparison to CFAR can be seen in Fig.~\ref{fig:comparsion_cfar_kstorng_normals}.
\begin{figure}
\vspace{0.2cm}
\begin{centering}
    \subfloat[CFAR keeps an excessive amount of points (black), including false positives, and surface points are poorly estimated.]
      {\includegraphics[trim={5cm 8.5cm 2cm 8cm},clip,width=0.9\hsize,angle=0]{figures/Filter/cfar.png}\label{fig:cfar_normals}}\\
    \subfloat[\ac{TITLE}: environment is represented by oriented surface points (red). The \textit{k-strongest} filtered points (fewer false positives) are shown in black.]
     {\includegraphics[trim={5cm 8.5cm 2cm 8cm},clip,width=0.9\hsize,angle=0]{figures/Filter/k_strongest.png}\label{fig:k_strong_normals}}
     \caption{Comparison of filtering methods, and oriented surface points.}
    \label{fig:comparsion_cfar_kstorng_normals}
 % \end{center}
  \end{centering}
  %\vspace{-0.2cm}
\end{figure}

\subsection{Multiple keyframe scan registration}
%\subsection{Scan registration procedure}
We employ a sliding window keyframe approach where the latest scan $\bm{\mathcal{M}}^t$ is registered to the $s$ most recent keyframes $\bm{\mathcal{M}}^{k_{1..s}}$. When the estimated relative pose %$||\mathbf{T}^{k_s-1}\mathbf{T}^{t}||$ 
exceeds a minimum rotation or translation to the latest keyframe, a new keyframe is stored from the current %sensors 
pose and point cloud $\{\bm{\mathcal{M}}^{k_s},\mathbf{T}^{k_s}\}\leftarrow\{\bm{\mathcal{M}}^t,\mathbf{T}^t\}$ and the oldest keyframe is removed. 
This ensures that drift is not introduced when the robot is stationary. Simultaneously registering to multiple keyframes can improve registration accuracy by imposing additional constraints, and improve robustness in cases when the registration is under-constrained or scan overlap drastically changes. Large changes in overlap can  occur due to occlusions from stationary or dynamic objects or due to non-planar road conditions~\cite{8917111}.% The method has similarities to~\cite{1642041}, except that

\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/Method/n_scan.png}
    \caption{The latest scan $\bm{\mathcal{P}}^t$ is registered to the $s=2$ previous key-frames. This can improve accuracy due to noise and robustness due to occlusions. }
    \label{fig:n_keyframe}
\end{figure}

We formulate the registration problem by minimizing a \textit{scan-to-keyframes (s2ks)} cost function %as seen in eq~\eqref{eq:reg}.
\begin{equation}
    \label{eq:reg}
    \underset{\mathbf{x}}{\mathrm{arg\: min}} f_{s2ks}(\bm{\mathcal{M}}^{k_{1..s}},\bm{\mathcal{M}}^t,\mathbf{x}),
\end{equation}
where we seek the transformation parameters
$\mathbf{x} \mathrel{\mathop:}= \begin{pmatrix} x & y & \theta\end{pmatrix}$ %$\mathbf{x}=[x \: y \: \theta]$ 
that best align the current scan $\bm{\mathcal{M}}^t$ with the key-frames $\bm{\mathcal{M}}^{k_{1..s}}$ jointly % as seen in eq~\eqref{eq:reg_individual}.

\begin{equation}
    \label{eq:reg_individual}
     f_{s2ks}(\bm{\mathcal{M}}^{k_{1..s}},\bm{\mathcal{M}}^t,\mathbf{x}) = \sum_{n=1}^{s}  f_{p2l}(\bm{\mathcal{M}}^{k_{n}},\bm{\mathcal{M}}^t,\mathbf{x}).
\end{equation}
The cost of aligning the latest scan $\bm{\mathcal{M}}^t$ to a single key-frame $\bm{\mathcal{M}}^k$ is given by the \textit{point-to-line (p2l)}~\cite{4543181} function $f_{p2l}$ in Eq.~\eqref{eq:scan_to_keyframe} .

\begin{equation}
    \label{eq:scan_to_keyframe}
    %\mathbf{\widetilde{\mu}}_t=
    %f_{p2l}(\mathcal{M}_{k_{n}},\mathcal{M}_t,\mathbf{x}) = \mathbf{n}_k \cdot \mathbf{p}^{\mu_k}_{\mu_t}
    f_{p2l}(\bm{\mathcal{M}}^k,\bm{\mathcal{M}}^t,\mathbf{x}) = \sum_{\forall i\in\bm{\mathcal{M}}^t} \mathcal{L}_\delta(\mathbf{n}^k_j \cdot (\mathbf{R}_{\theta}\bm{\mu}^t_i+\mathbf{t}_{x,y}-\bm{\mu}^k_j)),
     %\widetilde{n}_t=R(\theta)n_t
\end{equation}
where each surface point $i\in\bm{\mathcal{M}}^t$ is associated with the closest surface point $j\in\bm{\mathcal{M}}^k$ within a radius $r$ if the angle between the surface normals is within a tolerance $\theta_\mathrm{max}$. $\mathbf{R}_{\theta}$ and $\mathbf{t}_{x,y}$ is the rotation matrix and translation vector created from the optimization parameters. An intuition for the score is visualized in Fig.~\ref{fig:point_to_line}.

\begin{figure}
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.20\textwidth]{figures/Method/point2line.png}
    \caption{$\bm{\mathcal{M}}^t$ (blue) registered with $\bm{\mathcal{M}}^k$ (red). Most blue surface points (except one) have a correspondence with normals within $\theta_\mathrm{max}$ tolerance. The cost is given by the point-to-line distance visualized by black arrows.}
    \label{fig:point_to_line}
    \vspace{-0.2cm}
\end{figure}
Using the Huber loss $\mathcal{L}_\delta$, defined in Eq.~\eqref{eq:huber}, makes the cost less sensitive to outliers~\cite{Huber1992}. This is done by piecewise reshaping the cost function to increase quadratically for small values and linearly for larger values. 
\begin{equation}
    \label{eq:huber}
        \mathcal{L}_\delta(s)= 
\begin{cases}
    \frac{1}{2}s^2, & \text{if } |s|\leq \delta\\
    \delta(|s|-\frac{1}{2}\delta),              & \text{otherwise.}
\end{cases}
\end{equation}

We solve~\eqref{eq:reg} using the Broyden-Fletcher-Goldfarb-Shanno (BFGS) line search method with gradients obtained through automatic differentiation in the Ceres non-linear optimization framework~\cite{ceres-solver}.

\subsection{Accounting for motion}
%At each frame $t$ the previous pose $T_{t-1}$ and most recent velocity estimate $\{\mathbf{v}^{t-2}_{t-1},\omega^{t-2}_{t-1}\}$ was used to predict a starting point $\mathbf{x}_{init}$ for the optimization, and to compensate the filtered point cloud $\mathcal{P}_f$ from motion motion. This is important as the Navtech sensor operates at $4$hz.

At each frame the previous pose $\mathbf{T}^{t-1}$ and velocity estimate was used to predict a starting point $\mathbf{x}_\mathrm{init}$ for the optimization by linear extrapolation. The velocity was also used to compensate point cloud $\bm{\mathcal{P}}_f$ from motion distortion.
This is done by transforming all points into the time half way through the sweep, assuming that velocity is constant.



%\begin{equation}
%    \label{eq:reg_individual}
    %\mathbf{\widetilde{\mu}}_t=
    %p^{\mu_k}_{\mu_t} = (\mathbf{R}_{\theta}\mathbf{\mu}_t+\mathbf{t}_{x,y})-\mathbf{\mu}_\mu_k %(\mathbf{R}_{\theta}\mathbf{\mu}_t+\mathbf{t}_{x,y})-\mathbf{\mu}_\mu_k
     %\widetilde{n}_t=R(\theta)n_t
%\end{equation}







==> nykdtsnjtprfbjbpmwqncbnwxxgsfvcq/related_work.tex <==
%\subsection{Classical registraiton}
\label{sec:rw-lidar}\label{sec:rw-vision}
%Please give a brief introduction of the broad field of odometry estimation (ICP, NDT etc..) from the LIDAR and Vision perspective.


%\todo{Some range / vision stuff here:}
%Range based odometry commonly rely on incremental registration. The estimate can either be provided by aligning pairs of scans, e.g., the previous reading with the current one providing an incremental transformation which then are summed up to provide a current pose estimate. Many approaches are based on the iterative closest point (ICP) method, which consists of a typically rather expensive closest point search followed by a closed-form solution to obtain the next guess in the iteration. There are also alternatives that first compute a more compact representation, such as GMM or NDT which is used in the optimization formulation. With a few exceptions, for example, [Qianfang PAMI, take some more references there], registration is done through local search and to avoid that local minima are found, initial estimates from introceptive sensors as IMU and encoders are commonly used also together with a motion prediction step containing a motion model which accounts for kino-dynamic constraints. 

%For vision-based registration, there is the more classical approach of detecting features, which is used to handle correspondences between consecutive images, and to update the position of these features while estimating the motion of the vehicle. To provide a better estimate of the point features, several measurements are integrated into a local feature map. The utilization of local maps to improve dead reckoning in range data can also be utilized, ref? Another trending approaches is to rely on machine learning for handling correspondences (radar ref? + others) but also to obtain the full transformation (ref?). 

 

\subsection{Filtering radar data}
\label{sec:rw-filter}
%Introduction sentance

%Due to the characteristics of current radar systems, most radar odometry estimation systems are specifically designed to mitigate the effect of noise and reflections.
% CFAR etc, how can radar data be filtered.
%\cite{8813841} filters based dynamics using dopler data with front facing radar
% ~\cite{8794014} Week supervision that learns consistent features presents in both following radar images. (quite neat :) )
%\anas{
Raw radar scans are often converted to point clouds using filtering techniques that distinguish between targets and background noise. Due to the challenging noise characteristics of radar data, various approaches have been investigated to remove noise. The traditionally most widely used filtering technique, \ac{CFAR}~\cite{vivet2013localization}, cannot be applied directly, as it assumes known noise distribution \textit{a priori}, which is not the case with with \ac{FMCW} radar where reflections are context dependent. 
Moreover, \ac{CFAR} requires manual tuning of multiple parameters \cite{8793990,8460687}.
%In addition to that, it requires manual tuning for the threshold, number of training cells and the number of guard cells 

Another method is to simply set a fixed noise/signal threshold~\cite{mielle-2019-comparative}. However, doing so comes with the risk to remove important information since the noise background level varies greatly in different settings. 

Deep learning methods \cite{barnes_masking_2020,weston2019probably,8794014} have also been proposed for filtering but they require offline training and labeled data-sets as in \cite{barnes_masking_2020}. Wetson et al. \cite{weston2019probably} used lidar data for labeling, applying a static world assumption. Aldera et al. \cite{8794014} used sensor coherence and wheel odometry for training.
% 
In Marck et al.~\cite{marck2013indoor}, only the strongest power return per azimuth is kept. % and their filter removes beams if their neighbors produce errors in the range detection. 
In Fig.~\ref{fig:k_eval} we show that keeping only the strongest returns per azimuth is insufficient and makes the odometry estimation inaccurate. %Howvere, keeping only the strongest power return may also useful data.


In this work, we extend the work of Marck et al.~\cite{marck2013indoor} by including only the strongest $k$ returns in a given beam that exceed the expected noise level $\zmin$.
Section~\ref{ssec:Parameters} presents an experimental evaluation of the effect of $k$ %(and the noise threshold)
on the performance of radar odometry. A comparison between the proposed CFEAR filtering and the classical \ac{CFAR} method can be seen in Fig.~\ref{fig:k_threshold} and Fig.~\ref{fig:comparsion_cfar_kstorng_normals}.
%}
%\todo{Martin: Remember to include the following references}
%\cite{8460687} Precise Ego-Motion Estimation with Millimeter-Wave Radar under Diverse and Challenging Conditions

%\cite{8794014} uses weak supervision from an existing odometry estimator learns to filter incoherent measurements.

%\todo{Martin: do we want to add a plot here that shows how the signal from one beam might look, and the detections you'd get with CFAR, some fixed threshold, and k-max?}
\begin{figure}
	\input{figures/Parameters/figure_k_points}
	\caption{Typical power/range plot for a single azimuth reading. % using data from our quantitative evaluation.
	Here we use $k=12$ for conservative filtering that reduces false positives at the cost of missing some landmarks by simply limiting the maximum number of detections per azimuth. Accordingly, $\zmin$ can be selected low make the filter sensitive without drastically increase the number of false detections. In contrast, %cell-averaging
	\ac{CFAR} returns more spurious detections and is hard to tune.\label{fig:k_threshold}}
	\vspace{-0.3cm}
\end{figure}
%\todo{Anas - this is your show :)}


\subsection{Radar odometry}

%\begin{table}[]
%\begin{adjustbox}{width=\hsize}
%\begin{tabular}{l|lll}
%  Method & filter/landmark & association  &  matching &  \\
% Sarah H & Peaks+MPremoval  & largest subset with common shape  & Weighted Least squares SVD  &  \\
% Hong &  SURF  &  feature consistency+maximum inlier(clique) &  Least squares & Weighted Least squares SVD \\
 %Barnes Robust & Learned keypoints  & dense optimum keypoint search & Least squares SVD & 
%\end{tabular}
%\end{adjustbox}
%\end{table}


\label{sec:rw-radar}
Over the years, various methods have been proposed for radar SLAM~\cite{6689216, Vivet_2013, 7795967}.  Recent radar odometry methods can be divided into sparse methods that attempt to estimate keypoints or compute corresponding features from radar images, and dense methods that match a denser set of radar returns. % representing positive and negative information. (I this is actually cool and worth mention, what do you say?
Holder et al. used Iterative Closest Point (ICP) to align point clouds acquired from a front-facing radar~\cite{8813841} however the method relies on additional sensors.

Mielle et al.~\cite{mielle-2019-comparative} demonstrated radar odometry with off-the-shelf frameworks for range-based mapping in an indoor environment, using a fixed-threshold filtering method. 
However, the validation was done in a single, small-scale environment, and the fixed-threshold filtering has been found to be difficult to generalise to other environments. 

Cen et al. presented sparse methods for ego-motion~\cite{8460687,8793990}. A landmark extraction method detects peaks while removing multipath reflections. Data association and outlier rejection is carried out by finding the largest common subset of landmarks between subsequent scans. Landmarks are detected only in the polar space using 1d (power/range) signals. In contrast, our method additionally filters range data in Cartesian space and we obtain robustness to outliers via a Huber loss. Hong et al.~\cite{hong2020radarslam} proposed a full radar SLAM framework. The odometry method extract SURF feature descriptors without filtering the raw radar data and uses robust data association similarly to Cen~\cite{8460687}. 
Both Cen and Hong estimate egomotion by minimizing the (weighted) squared error between correspondences using SVD (Single Value Decomposition), the performance of their methods is included in our evaluation.


%Barnes and Posner~\cite{barnes_under_2020} proposed a self-supervised system for learning sparse robust key-points. A dense search is used to find correspondences.
%The method requires a substantial amount of training data, gathered over 250~km driving, and it's currently unclear how well the method generalizes to new spatial locations as no SCV (Spatial Cross Validation) was performed in the evaluation has been presented.

Barnes et al. presented two learning based methods for radar odometry.
In~\cite{barnes_masking_2020} a mask is learned for filtering dynamic objects and noise, matching is carried out by a dense correlation-based approach. Barnes and Posner later proposed a sparse method that learns keypoints, scores and descriptors for odometry and loop closure detection~\cite{barnes_under_2020}. Keypoints are associated via a dense search and matched by minimizing the squared distance using SVD. Both methods~\cite{barnes_masking_2020,barnes_under_2020} require supervision from a previously existing positioning system and an extensive amount of data collected over $200$~km driving. Spatial cross-validation shows that the accuracy drops by a factor of $2.4$ when estimating odometry in new streets not included in the training set, yet in nearby locations within the same city~\cite{barnes_masking_2020}. It is currently not known how well~\cite{barnes_under_2020} generalizes to new locations. Our method does not rely on training or a previously existing positioning system. In the evaluation we compare these methods to ours and qualitatively demonstrate how our method generalizes to widely different environments.



%Barnes et al. also presented~\cite{barnes_masking_2020}, a dense method that learns feature embeddings, that implicitly mitigate radar noise, for dense correlative scan matching. The method requires large amount of training data, collected over $216$km driving. Spatial cross validation show that the learned model generalizes to new locations within the same environment type (an urban environment), although with an error increased by roughly a factor~$2.4$.

Park et al.~\cite{9197231} used dense matching by applying the Fourier Mellin
transform (FMT) to Cartesian and log-polar radar images and estimating the relative motion from phase correlation in a course-to-fine fashion.
Their dense method yields slow run time performance and has not been compared to the state-of-the-art.

Radar odometry has also been improved by accounting for motion and Doppler distortion~\cite{burnett_we_2021}, using multiple Doppler radars~\cite{6907064} and by introspectively detecting registration failures~\cite{8917111}. Finally, radar based localization with respect to a map have also been proposed in~\cite{narula_all-weather_2020,saftescu_kidnapped_2020,gadd2020look,8957240,tang2020selfsupervised}. However, these methods are out of scope as we focus on the radar odometry problem without a prior map.

%\todo{Martin: Important to  cover also the citations in the last sentence, and to -- as clearly as possible -- relate your work to the references you cite here.}

